Algorithms for the local and the global postage stamp problem

We consider stamps with different values (denominations) and same dimensions, and an envelope with a fixed maximum number of stamp positions. The local postage stamp problem is to find the smallest value that cannot be realized by the sum of the stamps on the envelope. The global postage stamp problem is to find the set of denominations that maximize that smallest value for a fixed number of distinct denominations. The local problem is NP-hard and we propose here a novel algorithm that improves on both the time complexity bound and the amount of required memory. We also propose a polynomial approximation algorithm for the global problem together with its complexity analysis. Finally we show that our algorithms allow to improve secure multi-party computations on sets via a more efficient homomorphic evaluation of polynomials on ciphered values.

==> data_cover_k20_s0.tex <==
\begin{CacheMeCode}{gnuplot, cairolatex terminal={size 5.25,3.15 font "1" lw 2}}
set key left Left reverse
set title "denominations = 20"
set xlabel "stamps"
set ylabel 'speed-up vs \cite{Mossige:1981:hrange}'
set mxtics 2
set grid mxtics xtics
set ytics format '$10^{%T}$'

$Data << EOD
1 0.000002 0.000002 0.000002
2 0.000005 0.000005 0.000003
3 0.000020 0.000017 0.000010
4 0.000052 0.000049 0.000042
5 0.000224 0.000208 0.000239
6 0.000309 0.000198 0.000791
7 0.000837 0.000548 0.002864
8 0.001779 0.001200 0.008226
9 0.003409 0.002751 0.024922
10 0.005774 0.005546 0.069827
11 0.007070 0.006514 0.107836
12 0.007589 0.007683 0.154540
13 0.009103 0.008816 0.209938
14 0.009612 0.009990 0.273794
15 0.011131 0.011137 0.346455
16 0.012628 0.012255 0.426869
17 0.013113 0.013377 0.515895
18 0.014607 0.014515 0.613517
19 0.015184 0.015769 0.719494
20 0.016722 0.016892 0.833548
21 0.018214 0.018016 0.954977
22 0.018660 0.019119 1.085750
23 0.020181 0.020274 1.225220
24 0.020651 0.021373 1.371980
25 0.022151 0.022501 1.527440
26 0.023678 0.023615 1.690660
27 0.024304 0.024838 1.863120
28 0.025616 0.025871 2.043150
29 0.026136 0.027173 2.234310
30 0.027881 0.028128 2.430800
31 0.029099 0.029217 2.632680
32 0.029568 0.030329 2.844860
33 0.031062 0.031462 3.067450
34 0.031554 0.032585 3.295510
35 0.033022 0.033686 3.535610
36 0.034519 0.035133 3.786360
37 0.035036 0.036011 4.042450
38 0.036512 0.037058 4.297190
39 0.036965 0.038165 4.568370
40 0.038484 0.039286 4.843360
EOD

plot [1:] \
1 notitle with lines lc 3,\
$Data using 1:($4/$2) title '\cite{Mossige:1981:hrange}/\cref{alg:leo}' with linespoint lc 1 ps 0.5, \
$Data using 1:($4/$3) title '\cite{Mossige:1981:hrange}/\cref{alg:sliding}' with linespoint lc 2 ps 0.5
\end{CacheMeCode}
%$ %trick to end math eq

%plot \
%$Data using 1:4 title '\cite{Mossige:1981:hrange}' with linespoint lc 3 ps 0.5, \
%$Data using 1:2 title '\cref{alg:leo}' with linespoint lc 1 ps 0.5, \
%$Data using 1:3 title '\cref{alg:sliding}' with linespoint lc 2 ps 0.5


==> data_cover_k20_s1.tex <==
\begin{CacheMeCode}{gnuplot, cairolatex terminal={size 5.25,3.15 font "1" lw 2}}
set key left Left reverse
set title "denominations = 20, w. early-termination"
set xlabel "stamps"
set ylabel 'speed-up vs \cite{Mossige:1981:hrange}'
set mxtics 2
set grid mxtics xtics
set ytics format '$10^{%T}$'

$Data << EOD
1 0.000002 0.000003 0.000002
2 0.000005 0.000005 0.000003
3 0.000019 0.000016 0.000010
4 0.000050 0.000044 0.000042
5 0.000218 0.000187 0.000239
6 0.000312 0.000173 0.000789
7 0.000842 0.000484 0.002888
8 0.001770 0.001034 0.008259
9 0.003443 0.002349 0.024843
10 0.005951 0.004681 0.069592
11 0.007697 0.005973 0.106762
12 0.008516 0.007151 0.153173
13 0.010317 0.008292 0.208191
14 0.011071 0.009448 0.271745
15 0.012967 0.010705 0.343683
16 0.014677 0.011725 0.424157
17 0.015482 0.012969 0.512738
18 0.017232 0.013987 0.609798
19 0.018099 0.015231 0.715152
20 0.019877 0.016367 0.829145
21 0.021689 0.017486 0.951017
22 0.022420 0.018621 1.080760
23 0.024207 0.019738 1.219170
24 0.024967 0.020857 1.365940
25 0.026764 0.022006 1.521310
26 0.028527 0.023131 1.684290
27 0.029285 0.024246 1.856220
28 0.031089 0.025359 2.038230
29 0.031836 0.026502 2.223300
30 0.033570 0.027604 2.419760
31 0.035423 0.028740 2.623420
32 0.036130 0.029877 2.836270
33 0.037893 0.030980 3.057050
34 0.038701 0.032099 3.287630
35 0.040438 0.033253 3.523070
36 0.042201 0.034350 3.770360
37 0.043030 0.035481 4.022830
38 0.044732 0.036603 4.285010
39 0.045491 0.037726 4.555140
40 0.047326 0.038843 4.832400
EOD

plot [1:] \
1 notitle with lines lc 3,\
$Data using 1:($4/$2) title '\cite{Mossige:1981:hrange}/\cref{alg:leo}' with linespoint lc 1 ps 0.5, \
$Data using 1:($4/$3) title '\cite{Mossige:1981:hrange}/\cref{alg:sliding}' with linespoint lc 2 ps 0.5
\end{CacheMeCode}
%$ %trick to end math eq

%plot \
%$Data using 1:4 title '\cite{Mossige:1981:hrange}' with linespoint lc 3 ps 0.5, \
%$Data using 1:2 title '\cref{alg:leo}' with linespoint lc 1 ps 0.5, \
%$Data using 1:3 title '\cref{alg:sliding}' with linespoint lc 2 ps 0.5


==> data_cover_k35_s1.tex <==
\begin{CacheMeCode}{gnuplot, cairolatex terminal={size 5.5,2.1 font "1" lw 2}}
set key left Left reverse
set title "denominations = 35, with early-termination"
set xlabel "stamps"
set ylabel 'speed-up vs \cite{Mossige:1981:hrange}'
set mxtics 2
set grid mxtics xtics mytics ytics
#set ytics format '$10^{%T}$'

$Data << EOD
1 0.000003 0.000003 0.000002
2 0.000010 0.000009 0.000005
3 0.000068 0.000060 0.000034
4 0.000172 0.000115 0.000230
5 0.000934 0.000675 0.001595
6 0.002538 0.002288 0.009847
7 0.009967 0.007364 0.049159
8 0.029387 0.022967 0.207647
9 0.111741 0.090349 0.934987
10 0.330563 0.265037 3.694580
11 0.366002 0.302693 6.077300
12 0.421333 0.349593 9.043210
13 0.478786 0.397593 12.563200
14 0.534483 0.443158 16.640200
15 0.591461 0.490290 21.300100
16 0.647659 0.538650 26.482400
17 0.703626 0.585419 32.222000
18 0.761536 0.631611 38.536000
19 0.816217 0.681422 45.407200
20 0.871655 0.724697 52.810000
EOD


plot [1:15] \
1 notitle with lines lc 3,\
$Data using 1:($4/$2) title '\cite{Mossige:1981:hrange}/\cref{alg:leo}' with linespoint lc 1 pt 1 ps 0.5, \
$Data using 1:($4/$3) title '\cite{Mossige:1981:hrange}/\cref{alg:sliding}' with linespoint lc 2 pt 0ps 0.5
\end{CacheMeCode}
%$ %trick to end math eq


%$Data using 1:($6/$4) title 'OLD \cite{Mossige:1981:hrange}/\cref{alg:leo}' with linespoint lc 4 pt 8 ps 0.5, \
%$Data using 1:($6/$5) title 'OLD \cite{Mossige:1981:hrange}/\cref{alg:sliding}' with linespoint lc 7 pt 0 ps 0.5, \


==> data_cover_s05_s1.tex <==
\begin{CacheMeCode}{gnuplot, cairolatex terminal={size 5.5,2.1 font "1" lw 2}}
set key left Left reverse
set title "stamps = 5, with early-termination"
set xlabel "denominations"
set ylabel "seconds"
set mxtics 2
set ytics 0.1
set grid mxtics xtics
set ytics format '$10^{%T}$'

$Data << EOD
1 0.000002 0.000002 0.000002
2 0.000002 0.000002 0.000013
3 0.000002 0.000002 0.000003
4 0.000003 0.000003 0.000004
5 0.000004 0.000004 0.000005
6 0.000005 0.000005 0.000007
7 0.000007 0.000006 0.000009
8 0.000010 0.000010 0.000014
9 0.000013 0.000013 0.000016
10 0.000020 0.000017 0.000023
11 0.000026 0.000023 0.000028
12 0.000034 0.000029 0.000037
13 0.000048 0.000041 0.000051
14 0.000064 0.000056 0.000066
15 0.000075 0.000064 0.000083
16 0.000099 0.000084 0.000107
17 0.000123 0.000107 0.000130
18 0.000153 0.000131 0.000161
19 0.000193 0.000165 0.000204
20 0.000218 0.000187 0.000240
21 0.000256 0.000216 0.000298
22 0.000120 0.000087 0.000222
23 0.000146 0.000103 0.000274
24 0.000173 0.000122 0.000330
25 0.000209 0.000156 0.000376
26 0.000243 0.000179 0.000431
27 0.000295 0.000198 0.000518
28 0.000339 0.000226 0.000581
29 0.000406 0.000266 0.000697
30 0.000466 0.000326 0.000799
31 0.000528 0.000366 0.000936
32 0.000613 0.000414 0.001064
33 0.000698 0.000464 0.001192
34 0.000786 0.000519 0.001341
35 0.000932 0.000672 0.001594
36 0.001051 0.000748 0.001755
37 0.001133 0.000785 0.001952
38 0.001268 0.000861 0.002172
39 0.001487 0.001013 0.002518
40 0.001655 0.001117 0.002798
41 0.001794 0.001264 0.003004
42 0.002005 0.001412 0.003260
43 0.002263 0.001557 0.003687
44 0.002543 0.001746 0.004075
45 0.002871 0.001978 0.004640
46 0.003189 0.002197 0.005069
47 0.003435 0.002302 0.005459
48 0.003736 0.002531 0.005981
49 0.004362 0.003063 0.006788
50 0.004037 0.003155 0.008150
51 0.004638 0.003478 0.009063
52 0.005117 0.004041 0.009754
53 0.005711 0.004386 0.010784
54 0.006228 0.004711 0.011576
55 0.005864 0.005066 0.012713
56 0.006474 0.005369 0.013649
57 0.007198 0.005809 0.014477
58 0.008571 0.006654 0.015744
59 0.009479 0.007159 0.016995
60 0.010405 0.007679 0.018239
61 0.010409 0.007905 0.019989
62 0.011430 0.008488 0.021395
63 0.012790 0.009316 0.023782
64 0.013853 0.009891 0.025320
65 0.014427 0.010788 0.027192
66 0.015750 0.011595 0.028736
67 0.016314 0.012452 0.031075
68 0.017623 0.013250 0.032887
69 0.019451 0.014330 0.035547
70 0.019869 0.015293 0.037369
71 0.021659 0.016276 0.040137
72 0.024681 0.018012 0.042918
73 0.025953 0.019278 0.044981
74 0.028154 0.020491 0.047620
75 0.029486 0.021825 0.050751
76 0.031664 0.023083 0.054024
77 0.033211 0.024472 0.057296
78 0.035692 0.026032 0.060467
79 0.037579 0.027659 0.065350
80 0.040146 0.029110 0.068511
81 0.023869 0.017513 0.060714
82 0.025980 0.017989 0.063197
83 0.031960 0.023005 0.063278
84 0.029631 0.019640 0.070049
85 0.030157 0.021247 0.074809
86 0.032398 0.023041 0.078836
87 0.034797 0.024324 0.083739
88 0.036319 0.025528 0.087838
89 0.049281 0.036186 0.087801
90 0.039912 0.028134 0.096834
91 0.054347 0.040882 0.097029
92 0.046195 0.033508 0.106791
93 0.061221 0.045142 0.107295
94 0.051928 0.037627 0.117579
95 0.068062 0.050546 0.119421
96 0.058974 0.043175 0.131503
97 0.076254 0.056066 0.130376
98 0.064943 0.048697 0.142165
99 0.084041 0.061915 0.141902
100 0.072088 0.053602 0.157036
EOD

plot [1:] [0:0.35]\
$Data using 1:4 title '\cite{Mossige:1981:hrange}' with linespoint lc 3 pt 2 ps 0.5, \
$Data using 1:2 title '\cref{alg:leo}' with linespoint lc 1 pt 1 ps 0.5, \
$Data using 1:3 title '\cref{alg:sliding}' with linespoint lc 2 pt 0 ps 0.5
\end{CacheMeCode}
%$ %trick to end math eq


%$Data using 1:4 title 'OLD \cref{alg:leo}' with linespoint lc 4 pt 8 ps 0.5, \
%$Data using 1:5 title 'OLD \cref{alg:sliding}' with linespoint lc 7 pt 0 ps 0.5, \


==> data_cover_s10_s1.tex <==
\begin{CacheMeCode}{gnuplot, cairolatex terminal={size 5.5,2.1 font "1" lw 2}}
set key left Left reverse
set title "stamps = 10, with early-termination"
set xlabel "denominations"
set ylabel "seconds"
set mxtics 2
set grid mxtics xtics
set ytics format '$10^{%T}$'

$Data << EOD
1 0.000002 0.000002 0.000002
2 0.000014 0.000002 0.000014
3 0.000003 0.000003 0.000008
4 0.000005 0.000004 0.000016
5 0.000011 0.000008 0.000042
6 0.000023 0.000018 0.000095
7 0.000051 0.000038 0.000238
8 0.000096 0.000066 0.000519
9 0.000182 0.000129 0.000789
10 0.000399 0.000260 0.001590
11 0.000682 0.000429 0.003058
12 0.001067 0.000727 0.004748
13 0.000543 0.000273 0.003715
14 0.000908 0.000466 0.006138
15 0.001401 0.000689 0.009927
16 0.001742 0.001194 0.019073
17 0.002769 0.001733 0.024921
18 0.003319 0.002286 0.029887
19 0.004208 0.003247 0.043140
20 0.005939 0.004693 0.069621
21 0.007309 0.005474 0.097206
22 0.010565 0.007596 0.122068
23 0.014278 0.010205 0.166491
24 0.018265 0.014036 0.227079
25 0.024899 0.019064 0.294126
26 0.035140 0.026674 0.403535
27 0.045835 0.035925 0.540726
28 0.060609 0.047589 0.709544
29 0.077289 0.061056 0.894988
30 0.098338 0.077462 1.141320
31 0.124788 0.097117 1.481810
32 0.159201 0.125951 1.899710
33 0.205608 0.163560 2.336910
34 0.270172 0.213934 2.968680
35 0.330636 0.266276 3.698200
36 0.411442 0.327793 4.577890
37 0.517396 0.414844 5.773790
38 0.659692 0.525803 7.304760
39 0.775442 0.626653 8.679920
40 0.926324 0.741993 10.328400
EOD


plot [1:] \
$Data using 1:4 title '\cite{Mossige:1981:hrange}' with linespoint lc 3 pt 2 ps 0.5, \
$Data using 1:2 title '\cref{alg:leo}' with linespoint lc 1 pt 1 ps 0.5, \
$Data using 1:3 title '\cref{alg:sliding}' with linespoint lc 2 pt 0 ps 0.5
\end{CacheMeCode}
%$ %trick to end math eq

%$Data using 1:4 title 'OLD \cref{alg:leo}' with linespoint lc 4 pt 8 ps 0.5, \
%$Data using 1:5 title 'OLD \cref{alg:sliding}' with linespoint lc 7 pt 0 ps 0.5, \

